Exposure-Aware Informative Path Planning Using Deep Reinforcement Learning

This paper addresses the finite-budget exposure-aware informative path planning (IPP) problem for a fleet of mobile sensing agents. The agents map an unknown scalar field while limiting exposure to high field intensity. Existing IPP methods optimize informativeness under motion or resource constraints, but do not address field exposure constraints. We formulate exposure-aware IPP (EA-IPP) as a scalarized bi-objective belief-state Markov decision process that trades the normalized Gaussian-process (GP) information gain against a normalized measurement-derived fleet exposure index. A parameter-shared proximal policy optimization (PPO) framework with decentralized actors and a centralized fleet critic is trained offline and evaluated on unseen fields. Across the radar, plume, and wildfire field families, the EA-IPP agent achieves the lowest GP reconstruction RMSE among the evaluated baselines while retaining D-optimal information within $10\%$ of the non-learning information baseline. The minimum field exposure is approximately $34.6\%$, $20.1\%$, and $27\%$ below the non-exposure-aware baseline for radar, plume, and wildfire, respectively.

==> figure5/all_results.tex <==
% AUTO-GENERATED VERSION ENTRYPOINT -- safe to overwrite
% Data root: data5/


